Design Principles of Dynamic Resource Management for High-Performance Parallel Programming Models

With Dynamic Resource Management (DRM) the resources assigned to a job can be changed dynamically during its execution. From the system's perspective, DRM opens a new level of flexibility in resource allocation and job scheduling and therefore has the potential to improve system efficiency metrics such as the utilization rate, job throughput, energy efficiency, and responsiveness. From the application perspective, users can tailor the resources they request to their needs offering potential optimizations in queuing time or charged costs. Despite these obvious advantages and many attempts over the last decade to establish DRM in HPC, it remains a concept discussed in academia rather than being successfully deployed on production systems. This stems from the fact that support for DRM requires changes in all the layers of the HPC system software stack including applications, programming models, process managers, and resource management software, as well as an extensive and holistic co-design process to establish new techniques and policies for scheduling and resource optimization. In this work, we therefore start with the assumption that resources are accessible by processes executed either on them (e.g., on CPU) or controlling them (e.g., GPU-offloading). Then, the overall DRM problem can be decomposed into dynamic process management (DPM) and dynamic resource mapping or allocation (DRA). The former determines which processes (or which change in processes) must be managed and the latter identifies the resources where they will be executed. The interfaces for such \mbox{DPM/DPA} in these layers need to be standardized, which requires a careful design to be interoperable while providing high flexibility. Based on a survey of existing approaches we propose design principles, that form the basis of a holistic approach to DMR in HPC and provide a prototype implementation using MPI.

==> chapters/999_hierarchy.tex <==
\section{Hierarchical Interaction for Dynamic Resource Management}
\todo[inline]{Dominik@Martin Schulz: After some discussion (see below) we currently favor to include this Section somewhere in the end (e.g. between Discussion /Early Experiences and Summary). What do you think?}
\todo[inline]{Grenoble@Dominik: Without reading it first, this has to come last. First the principles, then the hierarchical approach.}
\todo[inline]{Dominik@Grenoble: I would argue that this is the frame in which our paradigms are embedded and thus needs to come first?}
\todo[inline]{Grenoble@Dominik: After reading it, it also just sounds obvious. This reads more like a proposal and what we discussed. It reminds me a lot of Flux :-).}
\todo[inline]{Dominik@Grenoble: Yes, it's obvious, yet noone (except Flux) seems to address it. It's not meant as a proposal but rather an abstract description of the reality of resource management on HPC systems. This paper could be a chance to promote thinking in an abstract hierarchy with a clear, generic interface between layers instead of "let's have some special interface between RM X and RTE Y, oh and we need yet another inteface for RTE Y and Programming Model Z and so on."}  
In this section we will show that Resource Management is inherently hierarchical (although often implicitly).
We provide formal definitions of terms and concepts of such a hierarchical setup, as any approach for dynamic resources is (implicitly or explicitly) embedded in such a setup. 
  
\textbf{1. (Dynamic) Resource Management is based on a directed control tree}
\begin{itemize}
	\item Dynamic Resource Management increases the complexity of resource management
	\begin{itemize}
		\item Higher frequency of decison making
		\item Larger parameter space for optimization
	\end{itemize}

	\item Deeper Control hierarchies can improve scalability
	\begin{itemize}
		\item Aggregation between levels
	\end{itemize}

	\item Typical HPC software stacks already build an implicit directed control tree where resource are assigned in a top-down approach
	\begin{itemize}
		\item Resource Manager: Optimizes efficiency of the whole system. Decides on (dynamic) resource allocations
		\item RTE/ Process Manager: Runs inside of a subset of a (dynamic) resource allocation. Thus its control lies inside of the (dynamic) resource allocation provided by the Resource Manager 
		\item Applications: Runs on a subset of resources manged by the PM. An applications control over resources is restricted to the resources assigne dto the application by the PM
	\end{itemize}	

	\item \textbf{Conclusion:} Dynamic Resources increase the need of deep directed tree-based control structures

	\item Notation: directed control tree $G_c = \{V_c, E_c\}$
	\begin{itemize}	
		\item The vertex $v^i_c$ represents a \textit{control component} (An instance of an control component possibly consists of multiple \textit{control agents}).
		\item The directed edge $e^k_c: v^i_c \rightarrow v^j_c$ indicates "control component $v^i_c$ assigns resources to control component $v^j_c$   
	\end{itemize}
\end{itemize}

\textbf{2. There exists a bijective mapping between the directed control tree $G_c = \{V_c, E_c\}$ and a directed resource tree $G_r=\{V_r,E_r\}$}
\begin{itemize}
	\item The vertex $v^i_r$ represent the resources controlled by control component $v^i_c$
	\item The edge $e^j_r$ represents the subset relation and can be associated with $e^j_c$, which translates to the meaning "Control component $v^i_c$ assigns a subset of its controlled resources to $v^j_c$".
\end{itemize}  

\textbf{3. Dynamic Resource Management requires a structure of information flow about resource requirements, in the inverse direction of the control tree}
	\begin{itemize}	
		\item Changing resources is subject to constraints, requirements and implications on the optimization objective
		\item These are specific to each control component
		\item This infomation is required by the parent control component as it restricts the space of possible reconfigurations of the children's resources
		\item This also restricts the space of possible reconfigurations of the parent components resources
		\item Thus, a transitive information flow from children to parents is required
		\item Infomation can be aggregated and transformed by a component before it is fowarded to its parent
	\end{itemize}



==> chapters/999_shortcomings.tex <==
\section{Shortcomings of previous approaches for dynamic resource management}
\label{sec:shortcomings}
In this section we highlight typical limitations of past approaches for dynamic resources in HPC which have so far prevented their adoption on production systems.

\textbf{Programming model specific approaches:} 
Many approaches target specific programming  models and therefor fail to establish a programming model agnostic standard interface for dynamic resources in HPC. 
A programming model agnostic interface is required to facilitate interoperability with the resource management software on the system.


\textbf{Granularity problem:}
A common limitations of many approaches is a too coarse grained granularity of resource changes.
Many approaches such as Elastic MPI, DMRlib and FlexMPI are based on adapting the MPI WORLD communicator to change the number of processes, i.e. a global synchronization across all processes of a job is required.
Besides obvious scalability concerns, this also significantly harms the flexibility of these approaches for jobs consisting of different, loosely-coupled parts such as task graph based applications or coupled simulations.
Therefor, a finer granularity than job-level granularity is required for a generic approach for dynamic resources. 

\textbf{MPI 2.0 Dynamic Process Management limitations:} 
Since MPI 2.0 the MPI Standard provides functionality for Dynamic Process Management (DPM). 
A central pillar of MPI DPM is the \lstinline{MPI_Comm_spawn} function. MPI Spawn is collective over an input communicator and provides functionalities to spawn new MPI processes at runtime.
The resulting intercommunicator connects the input communicator with a new MPI World communicator which contains the new MPI processes.
This approach ha

One problem is the blocking behavior of \lstinline{MPI_Comm_spawn}. This can lead to significant overheads as processes cannot continue their execution while new processes are launched.

Another problem is the connectedness of MPI processes created by a single invocation of MPI Spawn.
While processes from different \lstinline{MPI_COMM_WORLD} communicators can be disconnected with \lstinline{MPI_Comm_disconnect}, this is not possible for processes that share the same \lstinline{MPI_COMM_WORLD}. Therefore, the granularity in which MPI processes can be removed is restricted to the number of processes in the \lstinline{MPI_COMM_WORLD} communicators.
Approaches which try to overcome this issue by sequentially spawning single processes lead to high overheads for process spawning.

Finally, the specification of MPI Spawn does not describe the interaction with resource management software to change the current allocation.
Most implementations therefor default to spawning new processes inside of the current allocation, potentially oversubscribing resources.

Due to these limitations, approaches based on \lstinline{MPI_Comm_spawn} fall short of the performance and flexibility expected of a dynamic reosurce approach for HPC.

\textbf{Only either System-driven (malleability) or application-driven (evolving):}
Many approaches provide an interface for either system-driven changes of resources (malleability) or application-driven changes of resources (evolving).
Both approaches cannot reach optimal dynamic resource management due to a lack of local or global optimization information respectively.
Purely System-driven changes such as  lack information about application specifics such as reconfiguration points, data redistribution overheads, different application phases etc.
Although monitoring data can provide some insights into application behavior, a lot of optimization potential is lost due to a lack of information about the dynamic behavior of applications.
On the other hand, a purely application-driven approach, where applications request particular resources from the system lacks information about the global state of the system.
Therefor the system will not be able to optimize the global resource assignments based on such application-driven requests.
To globally optimize resource assignments in the system a cooperative approach between the Resource Manager and applications is required.

\textbf{Limited applicability to real-world applications}
So far, many approaches have only been demonstrated to work with particular application types (such as iterative solvers) or strongly simplified applications (benchmarks).
These applications are not representative for the large variety of HPC applications encountered on real systems and therefor cannot be deployed successfully on these systems.

\textbf{Lack of programmability:}
TODO
	
	
	
\begin{itemize}
	\item DMRlib, FlexMPI \cite{gonzalo13}, Adaptive MPI/Charm++/Maui-Torque \cite{prabhakaran15}, Invasive MPI (?), Elastic MPI \cite{compres16}, Charm++, Maui/Torque, COMPS, EasyGrid Application Management System, ReSHAPE.
	
	\item Main message: Hacks everywhere! Take what you have and hack down some prototype rather than an entirely new approach.
	
\end{itemize}

